CLARINET: A RISC-V Based Framework for Posit Arithmetic Empiricism

Many engineering and scientific applications require high precision arithmetic. IEEE~754-2008 compliant (floating-point) arithmetic is the de facto standard for performing these computations. Recently, posit arithmetic has been proposed as a drop-in replacement for floating-point arithmetic. The posit\texttrademark data representation and arithmetic claim several absolute advantages over the floating-point format and arithmetic, including higher dynamic range, better accuracy, and superior performance-area trade-offs. However, there does not exist any accessible, holistic framework that facilitates the validation of these claims of posit arithmetic, especially when the claims involve long accumulations (quire). In this paper, we present a consolidated general-purpose processor-based framework to support posit arithmetic empiricism. The end-users of the framework have the liberty to seamlessly experiment with their applications using posit and floating-point arithmetic since the framework is designed for the two number systems to coexist. Melodica is a posit arithmetic core that implements parametric fused operations that uniquely involve the quire data type. Clarinet is a Melodica-enabled processor based on the RISC-V ISA. To the best of our knowledge, this is the first-ever integration of quire with a RISC-V core. To show the effectiveness of the Clarinet platform, we perform an extensive application study and benchmark some of the common linear algebra and computer vision kernels. We emulate Clarinet on a Xilinx FPGA and present utilization and timing data. Clarinet and Melodica remain actively under development and is available in open-source for posit arithmetic empiricism.

==> quirebkp.tex <==
\noindent{\bf Numerical Examples:}

\begin{figure}[!h]
\centering
 \includegraphics[width=\columnwidth]{figures/numericalexamples.png}
\caption{Examples of accumulation and \emph{pi} calculation with posit, quire, and floating-point representation}
\label{fig:ieee754}
\end{figure}

Numerical examples of \texttt{pi} and \texttt{dot product} are shown in Fig.~\ref{fig:ieee754}. For \texttt{pi} calculation, 32-bit quire (q32) converges better compared to 32-bit posit (p32) or 32-bit floating-point (f32). In all our experiments, we have used 64-bit floating-point as a reference. For iteration 11 there is a dramatic increase in normalized error (compared to 64-bit floating-point) for \texttt{p32} and \texttt{f32}, but only a marginal increase in error for \texttt{q32}.  

In dot product, we use randomly generated vectors in the range of i) $2^0$ to $2^{-10}$, and ii) $2^0$ to $2^{-1000}$. We choose these ranges since the numbers are representable in all the formats. \texttt{q32} outperforms \texttt{p32}, \texttt{f32} and \texttt{q24}. Absolute error in \texttt{f32} is observed to be 9.9534475E-08, in \texttt{p32} it is 1.0127508E-08, in \texttt{q24} it is 8.14790212E-07, and in \texttt{q32} it is 2.676927E-09 in dot product of 10000 element vectors with the input data range of $2^0$ to $2^{-1000}$. The loss of precision in \texttt{q24} is close to one digit only while the reduction in the total bit-width is 8 bits compared to \texttt{f32}. The elaborated experiments on the dot product are depicted in section \ref{sec:blaslapack}. These preliminary experiments on pi calculation and dot product outline the superiority of using quire over 32-bit floating-point arithmetic. 
